Audio-Visual Synchronisation in the wild

In this paper, we consider the problem of audio-visual synchronisation applied to videos `in-the-wild' (ie of general classes beyond speech). As a new task, we identify and curate a test set with high audio-visual correlation, namely VGG-Sound Sync. We compare a number of transformer-based architectural variants specifically designed to model audio and visual signals of arbitrary length, while significantly reducing memory requirements during training. We further conduct an in-depth analysis on the curated dataset and define an evaluation metric for open domain audio-visual synchronisation. We apply our method on standard lip reading speech benchmarks, LRS2 and LRS3, with ablations on various aspects. Finally, we set the first benchmark for general audio-visual synchronisation with over 160 diverse classes in the new VGG-Sound Sync video dataset. In all cases, our proposed model outperforms the previous state-of-the-art by a significant margin.

==> fig_tab/Fig-class_stat.tex <==
\begin{figure}[!htb]
\centering
\includegraphics[width=1\textwidth]{images/data_sync.pdf}
\caption{Class ACC in VGG-Sound. TODO: chance is 9\%, show that as a horizontal line, also normalize the bar charts lower (e.g. 7\%) }
\vspace{-5mm}
\label{fig:class_stat}
\end{figure}


==> fig_tab/Fig-vgg_visual.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1\textwidth]{images/lrs_visual.pdf}
\vspace{2mm}
\caption{\textbf{Attention heatmaps on LRS3.} As expected, the model largely focuses on lip regions to the solve the task.}
\vspace{-5mm}
\label{fig:vgg_visual}
\end{figure}



==> fig_tab/Tab-noise_level.tex <==
\begin{table}[!htb]
\centering
\footnotesize
\begin{tabular}{lccccccc}
\toprule
Clip length 	    		& 5 	 & 10      & 15      & 20      & 25     & 30     \\\midrule
Visually evident     	& $50\%$ & $56\%$ & $$ & $62\%$  & $$ & $59\%$ \\ 
Uniform sound   	& $30\%$ & $35\%$ & $$ & $31\%$  & $$ & $38\%$ \\ 
No target sound/object & $20\%$ & $10\%$ & $$ & $7\%$  & $$ & $3\%$ \\ 
\bottomrule
\end{tabular}
\vspace{3mm}
\caption{\footnotesize  Noise in various length of sampled video clips}

\label{tab:noise}
\end{table}


==> fig_tab/Tab-result.tex <==
\begin{table}[!htb]
\centering
\footnotesize
\begin{tabular}{lccccccc}
\toprule
Method 	    & 5 	   & 7      & 9      & 11      & 13     & 15     \\\midrule
SyncNet     & $75.8$ & $82.3$ & $87.6$ & $91.8$  & $94.5$ & $96.1$ \\ 
PM    	    & $88.1$ & $93.8$ & $96.4$ & $97.9$  & $98.7$ & $99.1$ \\ 
Ours (fix) 	& $92.0$ & $95.5$ & $97.7$ & $98.8$  & $99.3$ & $99.6$ \\ 
Ours        & $91.9$ & $97.0$ & $98.8$ & $99.6$  & $99.8$ & $99.9$ \\\hdashline
\\
Ours + mask A   & $73.1$ & $85.3$ & $92.6$ & $96.1$  & $98.0$ & $99.2$ \\ 
Ours + mask V	& $76.5$ & $87.3$ & $93.4$ & $96.9$  & $98.2$ & $99.3$ \\ 
Ours + mask A,V & $71.7$ & $84.0$ & $91.2$ & $95.6$  & $97.7$ & $99.1$ \\ 
\bottomrule
\end{tabular}
\caption{\footnotesize  Audio-visual synchronization results on lrs2 dataset.}
\label{tab:results}
\end{table}


==> fig_tab/Tab-result_ablation.tex <==
\begin{table}[!htb]
\centering
\footnotesize
\begin{tabular}{lccccccc}
\toprule
Transformer depth  & 5 	    & 7      & 9      & 11      & 13     & 15     \\\midrule
PM     & $89.1$ & $94.0$ & $96.8$ & $98.4$  & $99.1$ & $99.4$ \\ 
Ours + 1 layer     & $89.1$ & $94.0$ & $96.8$ & $98.4$  & $99.1$ & $99.4$ \\ 
Ours + 2 layers	   & $91.6$ & $95.4$ & $97.6$ & $98.8$  & $99.9$ & $99.6$ \\ 
Ours + 3 layers    & $92.0$ & $95.5$ & $97.7$ & $98.8$  & $99.3$ & $99.6$ \\ 
\bottomrule
\end{tabular}
\caption{\footnotesize Ablation on the Transformer depth on the LRS2 dataset; as the Transformer depths increases, performance improves.}
\label{tab:results_abs}
\end{table}


==> fig_tab/Tab-result_ablations.tex <==
\begin{table}[!htb]
\footnotesize
\setlength\tabcolsep{4pt}
\begin{minipage}{.49\linewidth}
\centering
\begin{tabular}{lcccccc}
\toprule
Depth  & 5 	    & 7      & 9      & 11      & 13     & 15     \\\midrule
% PM-baseline    & $88.1$ & $93.8$ & $96.4$ & $97.9$  & $98.7$ & $99.1$ \\ 
1 layer     & $89.1$ & $94.0$ & $96.8$ & $98.4$  & $99.1$ & $99.4$ \\ 
2 layers	   & $91.6$ & $95.4$ & $97.6$ & $98.8$  & $99.1$ & $99.6$ \\ 
3 layers    & $92.0$ & $95.5$ & $97.7$ & $98.8$  & $99.3$ & $99.6$ \\ 
\bottomrule
\end{tabular}
\vspace{8pt}
\caption{\footnotesize \textbf{Ablation on Transformer depth (LRS2)}. Performance improves with more layers.}
\label{tab:depth}
\end{minipage}\hfill
\begin{minipage}{.49\linewidth}
\centering
\begin{tabular}{lccccccc}
\toprule
Mask	    & 5 	   & 7      & 9      & 11      & 13     & 15     \\\midrule
Audio   & $73.1$ & $85.3$ & $92.6$ & $96.1$  & $98.0$ & $99.2$ \\ 
Visual	& $76.5$ & $87.3$ & $93.4$ & $96.9$  & $98.2$ & $99.3$ \\ 
Both & $71.7$ & $84.0$ & $91.2$ & $95.6$  & $97.7$ & $99.1$ \\ 
\bottomrule
\end{tabular}
\vspace{8pt}
\caption{\footnotesize \textbf{Robustness test on LRS2.} 1 frame is masked for audio/visual/both modalities.}
\label{tab:robost}
\end{minipage}
\end{table}
% \captionsetup[subfloat]{labelformat=showtable}


==> fig_tab/Tab-result_arch.tex <==
\begin{table}[t]
\footnotesize
\RawFloats
\setlength\tabcolsep{1pt}
\begin{minipage}{.49\linewidth}
\centering
\renewcommand{\arraystretch}{1.62}
% \renewcommand{\arraystretch}{1}
\begin{tabular}{lccccccc}
\toprule
Method 	    & Var& 5 	   & 7      & 9      & 11      & 13     & 15     \\\midrule
% AVobjects &  $\times$  & $61.8$ & $72.0$ & $79.7$ & $85.4$  & $89.5$ & $91.8$ \\ 
\enc &  $\times$  & $70.2$ & $77.1$ & $83.3$ & $88.4$  & $92.0$ & $94.4$ \\
% \encmp 	& $\times$  & $78.6$ & $84.9$ & $89.8$ & $93.2$  & $95.5$ & $97.1$ \\ 
\encmp     & $\checkmark$   & $77.3$ & $88.0$ & $93.3$ & $96.4$  & $97.8$ & $98.6$ \\
\dec & $\checkmark$   & $75.7$ & $86.4$ & $89.4$ & $94.0$  & $95.1$ & $96.9$ \\

\bottomrule
\end{tabular}
\vspace{8pt}
\caption{\footnotesize \textbf{Effect of model variants on LRS3}. We use the `full-frame' dataset. `Var': whether models are trained and tested using variable length inputs. `5-15' refers to the number of input frames.}
\vspace{9pt}
\label{tab:results_arc}
\end{minipage}\hfill
\begin{minipage}{.49\linewidth}
\centering
\renewcommand{\arraystretch}{1.20}
\begin{tabular}{lcccccccc}
\toprule
Method 	    &\# Param& Var&5 	   & 7      & 9      & 11      & 13     & 15     \\\midrule
% \multicolumn{8}{c}{LRS2} \\
& & \multicolumn{2}{c}{LRS2} \\
\cmidrule(r r{1\tabcolsep}){3-4}   
% \cmidrule(c c{11pt}){3-4}     
% \cmidrule(c){3-4}
% \cdashline{1-8}
SyncNet~\cite{Chung16a}      &13.6M& $\times$&$75.8$ & $82.3$ & $87.6$ & $91.8$  & $94.5$ & $96.1$ \\ 
PM~\cite{chung2019perfect}     	   &13.6M& $\times$&$88.1$ & $93.8$ & $96.4$ & $97.9$  & $98.7$ & $99.1$ \\ 
% \encmp 	& $\times$&$92.0$ & $95.5$ & $97.7$ & $98.8$  & $99.3$ & $99.6$ \\ 
\encmp      &42.4M& $\checkmark$&$91.9$ & $97.0$ & $98.8$ & $99.6$  & $99.8$ & $99.9$ \\
% \cdashline{1-8}
\midrule
% \\
% \multicolumn{8}{c}{LRS3 ``full-frame''} \\
% & & \multicolumn{2}{c}{LRS3 ``full-frame''} \\
& & \multicolumn{2}{c}{LRS3} \\
\cmidrule(r r{1\tabcolsep}){3-4}     
% \cdashline{1-8}
AVobjects~\cite{Afouras20b} & 69.4M & $\times$  & $61.8$ & $72.0$ & $79.7$ & $85.4$  & $89.5$ & $91.8$ \\ 
\encmp     &42.4M & $\checkmark$   & $77.3$ & $88.0$ & $93.3$ & $96.4$  & $97.8$ & $98.6$ \\
\bottomrule
\end{tabular}
\vspace{5pt}
\caption{\footnotesize \textbf{Comparison to SOTA.} Synchronisation on LRS2 and LRS3 (``full-frame'').
% We outperform previous works by a large margin.
}
\label{tab:results_lrs2}
\end{minipage}
\vspace{-2mm}
\end{table}
% \captionsetup[subfloat]{labelformat=showtable}


